Extensions in Jacobian algebras via punctured skein relations

Given a Jacobian algebra arising from the punctured disk, we show that all non-split extensions can be found using the tagged arcs and skein relations previously developed in cluster algebras theory. Our geometric interpretation can be used to find non-split extensions over other Jacobian algebras arising form surfaces with punctures. We show examples in type $D$ and in a punctured surface.

==> respuesta_de_referee.tex <==
Specific comments to the authors:

⁃pp1, abstract, l4” form —> from  (hecho)

⁃pp2, right before Proposition: This phrase is not complete. Maybe say “… Jacobian algebras as made explicit in the next proposition” (hecho. no entendí mucho la sugerencia pero cambié la frase de todos modos)

⁃pp2. Proposition: perhaps say something like "a non-split triangle (not triangleS) with indecomposable extreme terms  $X_\alpha$ and $X_\beta$" (hecho)

⁃pp3, ln3: inecomposable —> indecomposable (hecho)

⁃	pp1, l11: I believe Brustle-Zhang introduced a geometric interpretation of Amiot’s generalized cluster categories, not defined them from scratch (cambiado. que hinchapelotas)


⁃	pp1, l(-4): if no frozen variables exist, by the decorated Teichmuller spaces associated to surfaces 
            (even in the presence of punctures), Ptolemy relations hold true by construction (hecho. que hinchapelotas)


      
⁃	pp2, Proposition: the condition in terms of dimension vectors being equal is already known in the literature in  such this is not a new result (aclaro que no lo encontramos en NINGUN lado en la introduccion)


⁃	pp3, Fig1: I presume the subscripts in the K’s indicate the position of the vector spaces K^j for j=1,2,3 but there is no remark regarding this. (agregada una frase sobre esto)
 

⁃	pp3, Lemma 2.2: Just to point out that this result is also illustrated for type D_5 in [Sch08], section 3.3.4.2  (agregado un remark sobre esto)       


⁃	pp4, after Fig.2: $I(a_n)$ should be $I(a_m)$ (cambiado)

- 19	⁃	pp13, §6: I think all of this section should made to an appendix as it does not contain any original result but only provide some examples (cambiado a medias)

pp4, Fig 2: the notation in part (b) is confusing and is not introduced (explicado)


 
 
2	⁃	pp5, sec 3.1: The authors consider cluster algebra elements here and refer to cluster expansion formulae of [MW13]. 
            However, they do not comment if the skein relations hold in the cluster algebra of the punctured disk. 
            If they only intend to consider smoothing representation theoretically in terms of non-split short exact sequences 
            or non-split triangles, the reference to [MW13] appears rather confusing
            (no se si lo resolvi porque no entiendo la pregunta)


            

3	⁃	pp5, Def 3.1: a new notation on the intersection number is introduced. This rather looks confusing and it is only introduced later in Def 3.2 which is puzzling for the reader if they do not notice it immediately (cambiado)


4	⁃	pp6, Fig 3: do you mean on the left? (cambiado)

 
5	⁃	pp6, l5: the notion of flip is not introduced (hecho)

6	⁃	pp7, Def 3.3: this definition and the example are not compatible; namely, what is referred to as left in part (1) appears to be right in Fig 5.  (cambiado)


7	⁃	pp7, Def 3.3: in part (2), it is not explained how the loop is obtained (no se si lo respondi pero trate)
 
8	⁃	pp 7, Fig 5: for type (4), the arcs gamma^{+}beta are missing and what is present in the figure appears to be \alpha^+\beta (hecho)


 
9	⁃	pp7, l(-1): say that the identities are in terms of cluster variables corresponding to the acs illustrated in the figure. 
            In particular these identities takes place in the cluster algebra

            (mas o menos cambiado)

10	⁃	pp8, a period is missing before Fig. 6. (hecho)


11	⁃	pp9, ln 1: in time? (cambiado)



12	⁃	pp9, §4, first para: Incomplete phrase (no entendi del todo pero cambie la oracion)


13	⁃	pp9, para2: before introducing the geometric realization of \tau, it is being referred and it is confusing for the reader. It is introduced right after but again this interrupts the flow (cambiado el orden)


14	⁃	pp9, papa2: not explained which direction rotation is considered (aclarada la direccion)

15	⁃	pp9, below Fig9: the notation of i \in [1,n-1] is confusing. Especially, what follows afterwards is incomprehensible (se saca esa notacion)

16	⁃	pp10, §4.2: the definition of smoothing is given again but this appears to be equivalent to the previous definition. 
            It only spells out a point of crossing in the definition so not clear what purpose this have
            (sacada la sobre explicacion)

17⁃	pp10-11, Fig 12-14: it appears that the main result of this paper is illustrated in figures 12 - 14 and the 
            middle terms of non-split s.e.s’s for arcs having two crossings are given by smoothing either one crossing point 
            (which give rise to the top three non-split extensions in Fig 14) or both of them (as given in Fig 14, part (9)). 
            It would be easier to see this correspondence visually if the points p,r,s,n are all consistent in all three figures (cambiado)

---------

---------      
 
 

 


        




            



            
18	⁃	pp 12, Lem 5.3, Prop 5.6: I am quite puzzled about this result since as far as I am concerned this is known in the 
            literature. The authors also indicate that the reference [CS17] in which a similar result is shown for unpunctured 
            surfaces but they do not give a similar characterization as in [CS17]. From my understanding, [CS17] 
            explicitly gives a characterization for such non-split s.e.s’s in the module category without 
            having to work in the cluster category 


———————————————————————————
* All references are from the manuscript

